Generating MIMO Channels For 6G Virtual Worlds Using Ray-tracing Simulations

Some 6G use cases include augmented reality and high-fidelity holograms, with this information flowing through the network. Hence, it is expected that 6G systems can feed machine learning algorithms with such context information to optimize communication performance. This paper focuses on the simulation of 6G MIMO systems that rely on a 3-D representation of the environment as captured by cameras and eventually other sensors. We present new and improved Raymobtime datasets, which consist of paired MIMO channels and multimodal data. We also discuss tradeoffs between speed and accuracy when generating channels via ray-tracing. We finally provide results of beam selection and channel estimation to assess the impact of the improvements in the ray-tracing simulation methodology.

==> definitions.tex <==
%This package must be friendly to all users at LASSE
%If a command is agressive to the template you are using, take it out, but comment in the gitlab log, so that other users will know what was excluded.
%For example, I (AK) moved all commands "\usepackage" to the file usepackages.tex.

%number of antenna elements
%\newcommand{\Nt}{N_{\mathrm{t}}}
%\newcommand{\Nr}{N_{\mathrm{r}}}
\newcommand{\Nt}{N_\mathrm{tx}}
\newcommand{\Nr}{N_\mathrm{rx}}

\def \Htk {{\bH_{t,k}}}
\def \Ht {{\bH_{t}}}

\newcommand{\Pts}[2] {{\Theta_{#1,#2}}}
%\def \Ptso {{\Theta_\textrm{t,s}}}

\newcommand {\arrowedbox}[1] {{\rightarrow\fbox{#1}\rightarrow}} %draw box with arrow

%Command "define" from http://www.latex-community.org/forum/viewtopic.php?f=46&t=15406
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\newcommand*{\defeqsmall}{\stackrel{\mathsmaller{\mathsf{def}}}{=}}

%use labels starting with eq: and fig: for equations and figures
\newcommand{\blol}[1] {{Block~(\ref{eq:#1})}}
\newcommand{\equl}[1] {{Eq.~(\ref{eq:#1})}}
\newcommand{\figl}[1] {{Fig.~\ref{fig:#1}}}
\newcommand{\tabl}[1] {{Table~\ref{tab:#1}}}
%use labels starting with ak_ for listings
\newcommand{\codl}[1] {{Listing~\ref{code:#1}}}
\newcommand{\exal}[1] {{Example~\ref{ex:#1}}}


%Expected value
\newcommand{\ev}{\mathbb{E}}

\renewcommand{\Re}{{\mathbb R}}
\newcommand{\ebt}{{\varepsilon_b}}
\newcommand{\eba}{{\overline\varepsilon_b}}
%\newcommand{\ekt}{{\varepsilon_k}}
\newcommand{\ekt}{\varepsilon_{\scriptscriptstyle K}}
\newcommand{\eka}{\overline\varepsilon_{\scriptscriptstyle K}}
\newcommand{\deck}{{F}}
\newcommand{\decb}{{f}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bt}{{\bf t}}
\renewcommand{\Re}{{\mathbb R}}
%\def \svmlight {{$\text{SVM}^{Light}$}}
\def \abM    {{$\alpha$~vs.~$\beta$}}
\def \svmlight {{$\text{SVM}^{Light}$}}
%\newcommand{\eka}{\overline\varepsilon_{\scriptscriptstyle K}}
%\def\x{{\mathbf x}}
%\def\L{{\cal L}}
%\def \abM    {{$\alpha$~vs~$\beta$}}
%\def \svmlight {{$\text{SVM}^{Light}$}}
%\newcommand{\Num} {\textrm{Num}}
%\newcommand{\Den} {\textrm{Den}}
%\newcommand{\tji} {{\theta_{ji}}}
%\newcommand{\tki} {{\theta_{ki}}}
%\newcommand{\aij} {{a_{ij}}}
%\newcommand{\Nji} {{N_{ji}}}
%\def \kernelxxi {\calK(\bx,\bx_i)}
%\newcommand{\sign} {\textrm{sign}}
%\newcommand{\bonea}{\overline{B_1}}
\newcommand{\ci}[1] {\textsf{#1}}
\newcommand{\co}[1] {\textsf{#1}}

\newcommand{\myattention}[1] {\textcolor{red}{\LARGE #1}}

\def \rvX     {{\bf X}}
\def \rvY     {{\bf Y}}
\newcommand {\Rd}      {{R^{d}}}
\newcommand {\Rg}      {{R^{g}}}
\newcommand {\Thetad}      {{\Theta^{d}}}
\newcommand {\Thetag}      {{\Theta^{g}}}

\newcommand{\bSigma}{\mbox{\boldmath$\Sigma$}}
\newcommand{\bmu}{\mbox{\boldmath$\mu$}}
\newcommand{\bpi}{\mbox{\boldmath$\pi$}}
\newcommand{\bnu}{\mbox{\boldmath$\nu$}}

%this one is beautiful for partial derivative:
\def \parder#1#2{{ \frac {\partial #1} {\partial #2}}}
%\def \tp#1#2#3{{\theta_{{#1 #2}}^{#3}}}
\newcommand{\tp}[3]{{\theta_{{#1 #2}}^{#3}}}

\ifdefined\bm
\else
\newcommand{\bm}[1]{{\mbox{\boldmath $#1$}}}
\fi

\newcommand{\Line}[0]{%
  \rule{0cm}{0cm}\\\hrule\rule{0cm}{0cm}%
}

%Alon Orlitsky
% Theorem-like environments

\def \qed     {\Box}  % here because other styles don't use box.

\ifdefined\Theorem
\else
\newtheorem{Theorem}{Theorem}
\fi

\newtheorem{Theorem*}{Theorem}

\newtheorem{Application}{Application}
\newtheorem{Application*}{Application}
\newtheorem{Claim}{Claim}
\newtheorem{Claim*}{Claim}

\ifdefined\Corollary
\else
\newtheorem{Corollary}[Theorem]{Corollary}
\fi

\newtheorem{CounterExample*}{$\overline{\hbox{\bf Example}}$}

\ifdefined\Example
\else
\newtheorem{Example}{Example}
\fi

\newtheorem{Example*}{Example}
\newtheorem{Exercise}{Exercise}
\newtheorem{Intuition*}{Intuition}
\newtheorem{Joke*}{Joke}

\ifdefined\Lemma
\else
\newtheorem{Lemma}[Theorem]{Lemma}
\fi


\newtheorem{Lemma*}{Lemma}
\newtheorem{Model}{Model}
\newtheorem{Model*}{Model}
\newtheorem{Open problem}{Open problem}
\newtheorem{Proposition}{Proposition}
\newtheorem{Property}{Property}
\newtheorem{Question}{Question}
\newtheorem{Question*}{Question}
\newtheorem{Remark*}{Remark}
\newtheorem{Result}{Result}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

%AK This has been redefined in dsl_definitions.tex in .\dslbook. If you need them
%copy and paste into your tex. Do not uncomment them here.
%\def \bApplication {\bthm{Application}}
%\def \eApplication {\ethm{Application}}
\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
%AK This has been redefined in dsl_definitions.tex in .\dslbook. If you need them
%copy and paste into your tex. Do not uncomment them here.
%\def \bExample   {\bthm{Example}}
%\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bModel     {\bthm{Model}}
\def \eModel     {\ethm{Model}}
\def \bOpen      {o\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
\def \bRemark    {\bthm{Remark}}
\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

\def \bSubexa    {\begin{subexa}}
\def \eSubexa    {\ethm{subexa}}

% Environments

\ifdefined\Problem
\else
\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\fi


\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{{}}

%\newcommand{\problem}[1]{#1}
%\newcommand{\problem}[1]{}

%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{{\bf Solution}\quad #1}
%\newcommand{\solution}[1]{#1}
%\newcommand{\solution}[1]{}

%\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}

% Formating

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Handouts

\newcommand{\hohead}[3]{
\hfill\begin{minipage}{3.5cm}
\bf
#1\\ % class # (CSE20) (perhaps + term)
#2\\ % term (Fall 2K+1) or name (Alon Orlitsky)
%Handout #3\\
\end{minipage}
}

\newcommand{\solhead}[3]{ % CSE20 -- Discrete Math; Fall 2K+1; 1
\begin{center}
  \Large #1\\[1ex]
  \normalsize #2\\[3ex]
  Solutions for Homework Assignment \##3\\
\end{center}
}

% Blackboard fonts

\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}} % \dN
\newcommand{\QQ}{\mathbb{Q}} % \dQ
\newcommand{\RR}{\mathbb{R}} % \dR
\newcommand{\ZZ}{\mathbb{Z}} % \dZ

% Numbers

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}
\newcommand{\RRp}{\reals^+}
\newcommand{\integersp}{\ZZ^+}
\newcommand{\integerss}[1]{\ZZ_{\ge{#1}}}

% boldface
\def \bzeroM {{\bf 0}}
\def \bff     {{\bf f}}

\def \bA {{\textbf A}}
\def \bB {{\textbf B}}
\def \bC {{\textbf C}}
\def \bD {{\textbf D}}
\def \bE {{\textbf E}}
\def \bF {{\textbf F}}
\def \bG {{\textbf G}}
\def \bH {{\textbf H}}
\def \bI {{\textbf I}}
\def \bJ {{\textbf J}}
\def \bK {{\textbf K}}
\def \bL {{\textbf L}}
\def \bM {{\textbf M}}
\def \bN {{\textbf N}}
\def \bO {{\textbf O}}
\def \bP {{\textbf P}}
\def \bQ {{\textbf Q}}
\def \bR {{\textbf R}}
\def \bS {{\textbf S}}
\def \bT {{\textbf T}}
\def \bU {{\textbf U}}
\def \bV {{\textbf V}}
\def \bW {{\textbf W}}
\def \bX {{\textbf X}}
\def \bY {{\textbf Y}}
\def \bZ {{\textbf Z}}

\def \ba {{\textbf a}}
\def \bb {{\textbf b}}
\def \bc {{\textbf c}}
\def \bd {{\textbf d}}
\def \be {{\textbf e}}
\def \bf {{\textbf f}}
\def \bg {{\textbf g}}
\def \bh {{\textbf h}}
\def \bi {{\textbf i}}
\def \bj {{\textbf j}}
\def \bk {{\textbf k}}
\def \bl {{\textbf l}}
\def \bm {{\textbf m}}
\def \bn {{\textbf n}}
\def \bo {{\textbf o}}
\def \bp {{\textbf p}}
\def \bq {{\textbf q}}
\def \br {{\textbf r}}
\def \bs {{\textbf s}}
\def \bt {{\textbf t}}
\def \bu {{\textbf u}}
\def \bv {{\textbf v}}
\def \bw {{\textbf w}}
\def \bx {{\textbf x}}
\def \by {{\textbf y}}
\def \bz {{\textbf z}}

\def \bmx {{\mathbf x}}

% caligraphics

\def \calA {{\cal A}}
\def \calB {{\cal B}}
\def \calC {{\cal C}}
\def \calD {{\cal D}}
\def \calE {{\cal E}}
\def \calF {{\cal F}}
\def \calG {{\cal G}}
\def \calH {{\cal H}}
\def \calI {{\cal I}}
\def \calJ {{\cal J}}
\def \calK {{\cal K}}
\def \calL {{\cal L}}
\def \calM {{\cal M}}
\def \calN {{\cal N}}
\def \calO {{\cal O}}
\def \calP {{\cal P}}
\def \calQ {{\cal Q}}
\def \calR {{\cal R}}
\def \calS {{\cal S}}
\def \calT {{\cal T}}
\def \calU {{\cal U}}
\def \calV {{\cal V}}
\def \calW {{\cal W}}
\def \calX {{\cal X}}
\def \calY {{\cal Y}}
\def \calZ {{\cal Z}}

\def \cala {{\cal a}}
\def \calb {{\cal b}}
\def \calc {{\cal c}}
\def \cald {{\cal d}}
\def \cale {{\cal e}}
\def \calf {{\cal f}}
\def \calg {{\cal g}}
\def \calh {{\cal h}}
\def \cali {{\cal i}}
\def \calj {{\cal j}}
\def \calk {{\cal k}}
\def \call {{\cal l}}
\def \calm {{\cal m}}
\def \caln {{\cal n}}
\def \calo {{\cal o}}
\def \calp {{\cal p}}
\def \calq {{\cal q}}
\def \calr {{\cal r}}
\def \cals {{\cal s}}
\def \calt {{\cal t}}
\def \calu {{\cal u}}
\def \calv {{\cal v}}
\def \calw {{\cal w}}
\def \calx {{\cal x}}
\def \caly {{\cal y}}
\def \calz {{\cal z}}

% vectors

%\def \veca  {{\overline a}}
%\def \vecb  {{\overline b}}
%\def \vecX  {{\overline X}}
%\def \vecY  {{\overline Y}}
%\def \vecx  {{\overline x}}
%\def \vecy  {{\overline y}}
%\def \vec#1{{\overline{#1}}}

% Abbreviations

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish

% notes

%\definecolor{light}{gray}{.75}

\def \mynote#1{{}}

% marginal notes

\def \marcha{{\marginpar{CHNGD}}}
\def \marfix{{\#\marginpar{FIX \#}}}
\def \marnew{{\marginpar{NEW}}}
\def \marok{{\#\marginpar{\# OK?}}}

% qed's

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}
\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \setpmo   {\{\pm 1\}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \set#1#2{{\{{#1}\upto{#2}\}}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \inseg#1{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations

%\def \union  {\cup}
\def \union  {\bigcup}
\def \unionl {\union\limits}
%\def \Union {\Bigcup} % want this
\def \Union  {\bigcup}
\def \Unionl {\Union\limits}

\def \inter  {\cap}
%\def \inter  {\bigcap}
\def \interl {\inter\limits}
\def \Inter {\Bigcap}
\def \Interl {\Inter\limits}

% Floors and Ceilings

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}

% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

\newcommand{\ed}{\stackrel{\mathrm{def}}{=}}
%\def \ed     {\,{\buildrel \rm def \over =}\,}
\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \pr     {{p}}
\def \Pr     {{\hbox{Pr}}}
\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

%\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions.
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

%\newcommand{\bi}{\begin{itemize}}
%\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

% for old documents

%\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
%\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{ % grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

